Quantifying Sensitivity for Tree Ensembles: A symbolic and compositional approach

Decision tree ensembles (DTE) are a popular model for a wide range of AI classification tasks, used in multiple safety critical domains, and hence verifying properties on these models has been an active topic of study over the last decade. One such verification question is the problem of sensitivity, which asks, given a DTE, whether a small change in subset of features can lead to misclassification of the input. In this work, our focus is to build a quantitative notion of sensitivity, tailored to DTEs, by discretizing the input space of the model and enumerating the regions which are susceptible to sensitivity. We propose a novel algorithmic technique that can perform this computation efficiently, within a certified error and confidence bound. Our approach is based on encoding the problem as an algebraic decision diagram (ADD), and further splitting it into subproblems that can be solved efficiently and make the computation compositional and scalable. We evaluate the performance of our technique over benchmarks of varying size in terms of number of trees and depth, comparing it against the performance of model counters over the same problem encoding. Experimental results show that our tool XCount achieves significant speedup over other approaches and can scale well with the increasing sizes of the ensembles.

==> regions.tex <==
We have presented an algorithm for counting the number of sensitive regions in decision tree ensembles
in contrast to the volume of the input space.
We follow the splits introduced by the trees to discretize the input space into regions.
However, our method can be extended to handle volume-based counting as well.
To achieve this, we can split the input space uniformly based on a predefined granularity for each feature such that all guard predicates align with the discretization.
Our method can then be applied to count the number of sensitive regions within this discretized space.
This approach allows us to approximate the volume of sensitive regions by counting the number of discretized regions
that fall within the sensitive areas.

Let us consider a feature $f$ with a range $[0, 1]$ and a granularity parameter $g_f = gcd(G_f+[0,1])$.
We discretize the range of features $f$ into intervals of size $g_f$, resulting in $\frac{1}{g_f}$ intervals.
For $k$th interval, we will assign internal bit $b_{fk}$.
The rest of encoding remains the same as described in Section~\ref{sec:prelim}. 

With this discretization, we provide a pathway to approximate volume-based sensitivity counting using our existing framework.
However, we have not taken this approach in our experiments as it increases the size of the discretized space significantly, leading to scalability issues if two guards are very close to each other.



% We can state the following theorem regarding the approximation guarantees of this approach.
% \begin{theorem}
% If we discretize each feature $f$ into intervals of size $g_f$, then the count of sensitive regions obtained using our method provides an approximation of the volume of sensitive regions.
% \end{theorem}











%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

